Single- and Multi-level Network Sparsification by Algebraic Distance

Network sparsification methods play an important role in modern network analysis when fast estimation of computationally expensive properties (such as the diameter, centrality indices, and paths) is required. We propose a method of network sparsification that preserves a wide range of structural properties. Depending on the analysis goals, the method allows to distinguish between local and global range edges that can be filtered out during the sparsification. First we rank edges by their algebraic distances and then we sample them. We also introduce a multilevel framework for sparsification that can be used to control the sparsification process at various coarse-grained resolutions. Based primarily on the matrix-vector multiplications, our method is easily parallelized for different architectures.

==> abstract.tex <==
\begin{abstract}
{%Computation in a reasonable time of such properties as the diameter, centrality indices, and  paths on networks may become the major bottleneck in the analysis if the network is big. Scalable approximation algorithms, heuristics and  structure preserving network sparsification methods play a crucial role in modern network analysis.
Network sparsification methods play an important role in modern network analysis when fast estimation of computationally expensive properties (such as the diameter, centrality indices, and paths) is required. 
%{Networks are often represented as graph data structures consisting of nodes that are linked by edges. This enables various algorithms to compute important properties of the network such as shortest paths, centrality indices and diameter. However, as the size of the network increases, computation of many of these properties in a realistic time frame becomes almost unattainable without scalable approximation algorithms, heuristics or network sparsification such that the sparse network becomes similar to the original one.} 
We propose a method of network sparsification that preserves a wide range of structural properties. Depending on the analysis goals, the method allows to distinguish between local and global range edges that can be filtered out during the sparsification. First we rank edges by their algebraic distances and then we sample them. We also introduce a multilevel framework for sparsification that can be used to control the sparsification process at various coarse-grained resolutions. 
Based primarily on the matrix-vector multiplications, our method is easily parallelized for different architectures.
%Finally, we show how our method can easily be parallelized for even faster runtimes.
}
{Networks, Sparsification, Multilevel Methods, Software, Scalable Algorithm}
%%%% If classification number provided then
%\\
%2000 Math Subject Classification: 34K30, 35K57, 35Q80,  92D25
\end{abstract}


==> prop-table.tex <==
\begin{table}[H]
	\footnotesize
	\centering
	\caption{Properties of fb-uf (FB), livejournal (LJ) and google-plus(Gplus)}\label{table:graph-properties}
	%\renewcommand{\arraystretch}{1.2}
	\begin{tabular}{|c|c|c|c|}                  %|c|c|
		\hline
		 &	FB & Gplus & LJ \\ \hline
		\begin{tabular}[x]{@{}c@{}} Clustering\\Coefficient \end{tabular} &	0.23 & 0.52 & 0.35	\\ \hline
		\begin{tabular}[x]{@{}c@{}} min/max/avg\\degree \end{tabular}	& 1/8246/83.49 & 1/20127/222.45 & 1/14815/17.35	\\ \hline
		Diameter	& 8 & 6 & 22 \\ \hline
		Modularity	& 0.45 & 0.48 & 0.74 \\
		\hline
	\end{tabular}
\end{table}

==> results/multiscale_results/bio_weak.tex <==
\begin{tabular}{ |l|l|l|l|l|l|l|l|l|l|l| }
		\hline
		\textbf{Graph Name} & \textbf{Level} & \multicolumn{9}{|c|}{ \textbf{Properties} } \\
		\hline
		- & - & \ $|E|$ & CC & D & Q & $\Gamma$ & $C_B$($\rho$) & $PR_{\rho}$ & $DC_{\rho}$ & $CC_{\rho}$\\
		\hline \multirow{4}{*}{bio-human-gene1}& G0 & 12.3M & 0.63 & 8.0 & 0.38 & 17 & 1.0 & 1.0 & 1.0 & 1.0\\
& G1 & 2.9M & 0.66 & 11.0 & 0.69 & 61 & 1.0 & 0.87 & 0.87 & 0.72\\
& G2 & 2.5M & 0.63 & 12.0 & 0.76 & 73 & 1.0 & 0.86 & 0.9 & 0.59\\
& G3 & 3.5M & 0.62 & 50.0 & 0.53 & 199 & 0.94 & 0.88 & 0.91 & 0.58\\
\hline
\multirow{4}{*}{bio-human-gene2}& G0 & 9.0M & 0.66 & 7.0 & 0.31 & 2 & 1.0 & 1.0 & 1.0 & 1.0\\
& G1 & 3.3M & 0.67 & 7.0 & 0.65 & 10 & 1.0 & 0.92 & 0.8 & 0.73\\
& G2 & 2.9M & 0.65 & 15.0 & 0.62 & 18 & 0.99 & 0.88 & 0.88 & 0.74\\
& G3 & 2.6M & 0.63 & 32.0 & 0.4 & 63 & 0.92 & 0.88 & 0.87 & 0.64\\
\hline
\multirow{4}{*}{bio-mouse-gene}& G0 & 14.5M & 0.53 & 12.0 & 0.62 & 97 & 1.0 & 1.0 & 1.0 & 1.0\\
& G1 & 3.8M & 0.58 & 16.0 & 0.92 & 98 & 0.99 & 0.94 & 0.94 & 0.71\\
& G2 & 4.0M & 0.5 & 15.0 & 0.77 & 114 & 0.99 & 0.92 & 0.91 & 0.67\\
& G3 & 3.4M & 0.41 & 13.0 & 0.78 & 97 & 1.0 & 0.89 & 0.89 & 0.6\\
\hline
\end{tabular}



==> results/multiscale_results/cit_weak.tex <==
\begin{tabular}{ |l|l|l|l|l|l|l|l|l|l|l| }
		\hline
		\textbf{Graph Name} & \textbf{Level} & \multicolumn{9}{|c|}{ \textbf{Properties} } \\
		\hline
		- & - & \ $|E|$ & CC & D & Q & $\Gamma$ & $C_B$($\rho$) & $PR_{\rho}$ & $DC_{\rho}$ & $CC_{\rho}$\\
		\hline \multirow{4}{*}{ca-cit-Hepth}& G0 & 2.4M & 0.61 & 9.0 & 0.41 & 74 & 1.0 & 1.0 & 1.0 & 1.0\\
& G1 & 515.9K & 0.71 & 13.0 & 0.94 & 125 & 0.99 & 0.82 & 0.85 & 0.74\\
& G2 & 505.0K & 0.7 & 18.0 & 0.8 & 307 & 0.99 & 0.77 & 0.85 & 0.64\\
& G3 & 471.9K & 0.52 & 40.0 & 0.65 & 2.1K & 0.99 & 0.68 & 0.84 & 0.09\\
\hline
\multirow{4}{*}{cit-patent}& G0 & 16.5M & 0.09 & 26.0 & 0.81 & 3.6K & 1.0 & 1.0 & 1.0 & 1.0\\
& G1 & 6.4M & 0.18 & 137.0 & 1.0 & 49.0K & 1.0 & 0.8 & 0.78 & 0.77\\
& G2 & 5.6M & 0.2 & 135.0 & 1.0 & 288.1K & 1.0 & 0.73 & 0.75 & 0.71\\
& G3 & 4.5M & 0.09 & 107.0 & 0.99 & 723.1K & 1.0 & 0.57 & 0.66 & 0.59\\
\hline
\multirow{4}{*}{codblp}& G0 & 15.2M & 0.82 & 23.0 & 0.84 & 1 & 1.0 & 1.0 & 1.0 & 1.0\\
& G1 & 6.0M & 0.95 & 23.0 & 1.0 & 36.1K & 1.0 & 0.5 & 0.78 & 0.56\\
& G2 & 3.5M & 0.9 & 30.0 & 1.0 & 71.6K & 1.0 & 0.22 & 0.53 & 0.51\\
& G3 & 4.1M & 0.59 & 45.0 & 0.99 & 73.2K & 1.0 & 0.27 & 0.67 & 0.14\\
\hline
\end{tabular}



==> results/multiscale_results/ms_result_table.tex <==
\begin{tabular}{ |l|l|l|l|l|l|l|l|l|l|l| }
\hline
Graph & Hierarchy & \multicolumn{9}{|c|}{ Properties } \\
\hline
- & - & $|E|$ & CC & Diameter & Q & $\Gamma_c$ & $C_B$ ($\rho$) & $P_R$ ($\rho$) & $C_{D}$ ($\rho$) & CC ($\rho$)\\
\hline \multirow{4}{*}{fb-indiana}& Original G0 & 1305757 & 0.2085 & 8.0 & 0.4444 & 1 & 1.0 & 1.0 & 1.0 & 1.0\\
& Coarse G1 & 462238 & 0.3023 & 10.0 & 0.8925 & 17 & 0.9966 & 0.8679 & 0.8389 & 0.689\\
& Mid G2 & 519070 & 0.2793 & 20.0 & 0.6869 & 25 & 0.9931 & 0.8844 & 0.8533 & 0.7\\
& Fine G3 & 237413 & 0.2853 & 51.0 & 0.7859 & 735 & 0.9856 & 0.8104 & 0.848 & 0.2747\\
\hline
\multirow{4}{*}{fb-uf}& Original G0 & 1465654 & 0.225 & 8.0 & 0.4375 & 1 & 1.0 & 1.0 & 1.0 & 1.0\\
& Coarse G1 & 407203 & 0.3467 & 11.0 & 0.9197 & 26 & 0.9973 & 0.8355 & 0.8294 & 0.6118\\
& Mid G2 & 569159 & 0.299 & 25.0 & 0.6609 & 38 & 0.9955 & 0.8919 & 0.8248 & 0.6761\\
& Fine G3 & 269303 & 0.3067 & 43.0 & 0.8009 & 1157 & 0.9815 & 0.7868 & 0.8401 & 0.2535\\
\hline
\multirow{4}{*}{codblp}& Original G0 & 15245729 & 0.8152 & 23.0 & 0.8432 & 1 & 1.0 & 1.0 & 1.0 & 1.0\\
& Coarse G1 & 5977964 & 0.9464 & 23.0 & 0.9982 & 36055 & 0.9995 & 0.5018 & 0.7831 & 0.5586\\
& Mid G2 & 3510715 & 0.9014 & 30.0 & 0.9987 & 71639 & 0.9995 & 0.2167 & 0.5346 & 0.5082\\
& Fine G3 & 4058906 & 0.5947 & 45.0 & 0.9934 & 73156 & 0.9995 & 0.275 & 0.6706 & 0.1431\\
\hline
\multirow{4}{*}{buzznet}& Original G0 & 2763066 & 0.2508 & 5.0 & 0.3101 & 1 & 1.0 & 1.0 & 1.0 & 1.0\\
& Coarse G1 & 959684 & 0.2949 & 13.0 & 0.6323 & 14 & 0.9994 & 0.6508 & 0.8643 & 0.4969\\
& Mid G2 & 669980 & 0.2956 & 23.0 & 0.6684 & 51 & 0.9974 & 0.6283 & 0.8914 & 0.5041\\
& Fine G3 & 758087 & 0.2538 & 34.0 & 0.6022 & 1063 & 0.9966 & 0.5748 & 0.8895 & 0.3507\\
\hline
\multirow{4}{*}{blogcatalog}& Original G0 & 2093195 & 0.4578 & 9.0 & 0.318 & 1 & 1.0 & 1.0 & 1.0 & 1.0\\
& Coarse G1 & 453344 & 0.4776 & 10.0 & 0.8149 & 19 & 0.9972 & 0.7964 & 0.8423 & 0.5017\\
& Mid G2 & 785275 & 0.4841 & 20.0 & 0.6435 & 14 & 0.9935 & 0.8842 & 0.925 & 0.6698\\
& Fine G3 & 659981 & 0.4647 & 19.0 & 0.6412 & 509 & 0.9947 & 0.749 & 0.8858 & 0.4104\\
\hline
\multirow{4}{*}{flickr}& Original G0 & 2316948 & 0.0894 & 9.0 & 0.6748 & 83 & 1.0 & 1.0 & 1.0 & 1.0\\
& Coarse G1 & 915654 & 0.1429 & 35.0 & 0.9181 & 140 & 0.9979 & 0.6002 & 0.6216 & 0.781\\
& Mid G2 & 756445 & 0.1337 & 36.0 & 0.8878 & 220 & 0.9974 & 0.6541 & 0.6885 & 0.8211\\
& Fine G3 & 603179 & 0.1652 & 49.0 & 0.8397 & 10499 & 0.9977 & 0.6081 & 0.7153 & 0.7334\\
\hline
\multirow{4}{*}{catster}& Original G0 & 5448197 & 0.4055 & 10.0 & 0.3926 & 281 & 1.0 & 1.0 & 1.0 & 1.0\\
& Coarse G1 & 1401552 & 0.3097 & 12.0 & 0.7832 & 296 & 0.999 & 0.709 & 0.6424 & 0.4156\\
& Mid G2 & 1083025 & 0.3447 & 23.0 & 0.7094 & 408 & 0.9989 & 0.6583 & 0.5491 & 0.6475\\
& Fine G3 & 969205 & 0.2607 & 38.0 & 0.7515 & 2641 & 0.9956 & 0.6572 & 0.6974 & 0.457\\
\hline
\multirow{4}{*}{bio-human2}& Original G0 & 9027024 & 0.6574 & 7.0 & 0.3124 & 2 & 1.0 & 1.0 & 1.0 & 1.0\\
& Coarse G1 & 3308311 & 0.6726 & 7.0 & 0.647 & 10 & 0.996 & 0.9229 & 0.7971 & 0.726\\
& Mid G2 & 2940587 & 0.6481 & 15.0 & 0.6218 & 18 & 0.9948 & 0.8843 & 0.8814 & 0.7405\\
& Fine G3 & 2588045 & 0.628 & 32.0 & 0.3977 & 63 & 0.9242 & 0.8838 & 0.8659 & 0.6414\\
\hline
\multirow{4}{*}{fb-penn94}& Original G0 & 1362220 & 0.2174 & 8.0 & 0.4875 & 1 & 1.0 & 1.0 & 1.0 & 1.0\\
& Coarse G1 & 520053 & 0.304 & 13.0 & 0.8562 & 19 & 0.997 & 0.8821 & 0.7634 & 0.6711\\
& Mid G2 & 385449 & 0.315 & 40.0 & 0.7896 & 170 & 0.9925 & 0.8368 & 0.81 & 0.5293\\
& Fine G3 & 381691 & 0.2848 & 35.0 & 0.771 & 1213 & 0.9925 & 0.8132 & 0.8394 & 0.2704\\
\hline
\multirow{4}{*}{ca-cit-Hepth}& Original G0 & 2444798 & 0.6117 & 9.0 & 0.4132 & 74 & 1.0 & 1.0 & 1.0 & 1.0\\
& Coarse G1 & 515851 & 0.7127 & 13.0 & 0.9437 & 125 & 0.9935 & 0.8235 & 0.8533 & 0.7424\\
& Mid G2 & 505024 & 0.6987 & 18.0 & 0.7991 & 307 & 0.9924 & 0.7724 & 0.8524 & 0.6441\\
& Fine G3 & 471865 & 0.5183 & 40.0 & 0.6518 & 2145 & 0.9852 & 0.6845 & 0.837 & 0.085\\
\hline
\multirow{4}{*}{livemocha}& Original G0 & 2193083 & 0.0582 & 6.0 & 0.3558 & 1 & 1.0 & 1.0 & 1.0 & 1.0\\
& Coarse G1 & 817527 & 0.065 & 12.0 & 0.6567 & 6 & 0.9981 & 0.8973 & 0.885 & 0.5863\\
& Mid G2 & 501243 & 0.0653 & 36.0 & 0.7482 & 12 & 0.9906 & 0.8338 & 0.8539 & 0.4837\\
& Fine G3 & 414197 & 0.0509 & 28.0 & 0.6763 & 1420 & 0.9924 & 0.7436 & 0.8635 & 0.4043\\
\hline
\multirow{4}{*}{fb-texas84}& Original G0 & 1590651 & 0.1974 & 7.0 & 0.374 & 1 & 1.0 & 1.0 & 1.0 & 1.0\\
& Coarse G1 & 558323 & 0.2576 & 11.0 & 0.8005 & 10 & 0.9965 & 0.8965 & 0.8982 & 0.6827\\
& Mid G2 & 495728 & 0.2528 & 19.0 & 0.6656 & 47 & 0.9944 & 0.8831 & 0.827 & 0.6121\\
& Fine G3 & 270594 & 0.2368 & 31.0 & 0.6914 & 971 & 0.992 & 0.8246 & 0.8451 & 0.1868\\
\hline
\multirow{4}{*}{livejournal}& Original G0 & 34681189 & 0.3538 & 21.0 & 0.75 & 1 & 1.0 & 1.0 & 1.0 & 1.0\\
& Coarse G1 & 13806113 & 0.4611 & 61.0 & 0.9972 & 1324 & 0.9999 & 0.8603 & 0.8206 & 0.7556\\
& Mid G2 & 11669864 & 0.4586 & 94.0 & 0.9523 & 69335 & 0.9999 & 0.8587 & 0.8314 & 0.7277\\
& Fine G3 & 10278150 & 0.2219 & 64.0 & 0.8819 & 563696 & 0.9999 & 0.6723 & 0.7449 & 0.3697\\
\hline
\multirow{4}{*}{gplus}& Original G0 & 12238285 & 0.5165 & 6.0 & 0.4754 & 1 & 1.0 & 1.0 & 1.0 & 1.0\\
& Coarse G1 & 3329596 & 0.5476 & 13.0 & 0.9143 & 34 & 0.999 & 0.9084 & 0.901 & 0.5887\\
& Mid G2 & 4714192 & 0.5209 & 20.0 & 0.7247 & 121 & 0.9987 & 0.9149 & 0.8934 & 0.6373\\
& Fine G3 & 2764745 & 0.4074 & 62.0 & 0.7077 & 3602 & 0.9952 & 0.7898 & 0.8544 & -0.0516\\
\hline
\multirow{4}{*}{bio-mouse}& Original G0 & 14461095 & 0.5308 & 12.0 & 0.6173 & 97 & 1.0 & 1.0 & 1.0 & 1.0\\
& Coarse G1 & 3841155 & 0.5782 & 16.0 & 0.925 & 98 & 0.9935 & 0.9371 & 0.9431 & 0.711\\
& Mid G2 & 4045880 & 0.5035 & 15.0 & 0.7668 & 114 & 0.9947 & 0.9212 & 0.9137 & 0.6679\\
& Fine G3 & 3415333 & 0.4071 & 13.0 & 0.7837 & 97 & 0.9953 & 0.892 & 0.892 & 0.6022\\
\hline
\multirow{4}{*}{cit-patent}& Original G0 & 16518947 & 0.0919 & 26.0 & 0.8127 & 3627 & 1.0 & 1.0 & 1.0 & 1.0\\
& Coarse G1 & 6424260 & 0.1814 & 137.0 & 0.9998 & 49041 & 0.9999 & 0.7954 & 0.7801 & 0.7703\\
& Mid G2 & 5554873 & 0.1956 & 135.0 & 0.9988 & 288120 & 0.9999 & 0.7285 & 0.7515 & 0.7134\\
& Fine G3 & 4452683 & 0.0912 & 107.0 & 0.9949 & 723056 & 0.9999 & 0.5678 & 0.6618 & 0.5852\\
\hline
\multirow{4}{*}{bio-human1}& Original G0 & 12323680 & 0.6303 & 8.0 & 0.3832 & 17 & 1.0 & 1.0 & 1.0 & 1.0\\
& Coarse G1 & 2892887 & 0.6633 & 11.0 & 0.6914 & 61 & 0.9968 & 0.8724 & 0.8743 & 0.7154\\
& Mid G2 & 2453881 & 0.6319 & 12.0 & 0.7562 & 73 & 0.9966 & 0.8616 & 0.8974 & 0.5886\\
& Fine G3 & 3465963 & 0.6162 & 50.0 & 0.5267 & 199 & 0.939 & 0.8847 & 0.9069 & 0.5842\\
\hline
\multirow{4}{*}{foursquare}& Original G0 & 3214986 & 0.2209 & 4.0 & 0.4029 & 1 & 1.0 & 1.0 & 1.0 & 1.0\\
& Coarse G1 & 1174157 & 0.1722 & 32.0 & 0.936 & 23 & 0.9997 & 0.6949 & 0.8711 & 0.8648\\
& Mid G2 & 1207313 & 0.1908 & 42.0 & 0.8615 & 26 & 0.9989 & 0.6954 & 0.8705 & 0.866\\
& Fine G3 & 1139482 & 0.2176 & 32.0 & 0.7568 & 7509 & 0.9995 & 0.5685 & 0.8098 & 0.8339\\
\hline
\end{tabular}


==> results/multiscale_results/ms_result_table2.tex <==
\begin{tabular}{ |l|l|l|l|l|l|l|l|l|l|l| }
\hline
Graph Name & Graphs & \multicolumn{9}{|c|}{ Properties } \\
\hline
- & - & \#Edges & Clustering Coefficient & Diameter & Modularity & Components & Betweenness ($\rho$) & Pagerank ($\rho$) & Degree Centrality ($\rho$) & Clustering Coefficient ($\rho$)\\
\hline \multirow{4}{*}{fb-indiana}& Original G0 & 1305757 & 0.2085 & 8.0 & 0.4461 & 1 & 1.0 & 1.0 & 1.0 & 1.0\\
& Coarse G1 & 361350 & 0.3146 & 13.0 & 0.9338 & 18 & 0.9963 & 0.8442 & 0.8289 & 0.6438\\
& Mid G2 & 349809 & 0.1441 & 10.0 & 0.336 & 8 & 0.9932 & 0.8892 & 0.8941 & 0.5673\\
& Fine G3 & 402723 & 0.0403 & 12.0 & 0.304 & 37 & 0.9932 & 0.9255 & 0.9454 & 0.0327\\
\hline
\multirow{4}{*}{fb-uf}& Original G0 & 1465654 & 0.225 & 8.0 & 0.4445 & 1 & 1.0 & 1.0 & 1.0 & 1.0\\
& Coarse G1 & 423369 & 0.2398 & 12.0 & 0.6072 & 3 & 0.994 & 0.8836 & 0.8818 & 0.583\\
& Mid G2 & 425060 & 0.1609 & 11.0 & 0.3665 & 15 & 0.9954 & 0.8967 & 0.9015 & 0.5981\\
& Fine G3 & 418930 & 0.0503 & 11.0 & 0.2703 & 57 & 0.9953 & 0.9228 & 0.9476 & -0.0128\\
\hline
\multirow{4}{*}{codblp}& Original G0 & 15245729 & 0.8152 & 23.0 & 0.8418 & 1 & 1.0 & 1.0 & 1.0 & 1.0\\
& Coarse G1 & 5294209 & 0.9109 & 30.0 & 0.9823 & 20068 & 0.9991 & 0.5484 & 0.7772 & 0.6802\\
& Mid G2 & 3368857 & 0.8094 & 32.0 & 0.9715 & 44276 & 0.9992 & 0.267 & 0.6262 & 0.6167\\
& Fine G3 & 4695002 & 0.5031 & 29.0 & 0.8393 & 29060 & 0.9991 & 0.515 & 0.8248 & 0.3805\\
\hline
\multirow{4}{*}{buzznet}& Original G0 & 2763066 & 0.2508 & 5.0 & 0.3133 & 1 & 1.0 & 1.0 & 1.0 & 1.0\\
& Coarse G1 & 713832 & 0.2626 & 11.0 & 0.502 & 1 & 0.9988 & 0.8231 & 0.9055 & 0.601\\
& Mid G2 & 919287 & 0.2089 & 18.0 & 0.2962 & 12 & 0.9989 & 0.8327 & 0.942 & 0.6024\\
& Fine G3 & 666569 & 0.1033 & 16.0 & 0.2863 & 239 & 0.9986 & 0.745 & 0.8944 & 0.2756\\
\hline
\multirow{4}{*}{blogcatalog}& Original G0 & 2093195 & 0.4578 & 9.0 & 0.3179 & 1 & 1.0 & 1.0 & 1.0 & 1.0\\
& Coarse G1 & 423884 & 0.4058 & 14.0 & 0.6704 & 1 & 0.9967 & 0.8096 & 0.869 & 0.4695\\
& Mid G2 & 570765 & 0.2613 & 11.0 & 0.2671 & 9 & 0.9975 & 0.8486 & 0.887 & 0.4417\\
& Fine G3 & 566093 & 0.1834 & 12.0 & 0.2348 & 391 & 0.9973 & 0.7005 & 0.8348 & 0.2907\\
\hline
\multirow{4}{*}{flickr}& Original G0 & 2316948 & 0.0894 & 9.0 & 0.6748 & 83 & 1.0 & 1.0 & 1.0 & 1.0\\
& Coarse G1 & 921040 & 0.1499 & 35.0 & 0.9111 & 144 & 0.9981 & 0.5974 & 0.6244 & 0.7818\\
& Mid G2 & 496077 & 0.1171 & 18.0 & 0.8423 & 134 & 0.997 & 0.7052 & 0.7285 & 0.7975\\
& Fine G3 & 634942 & 0.0374 & 25.0 & 0.546 & 5834 & 0.9965 & 0.6354 & 0.7689 & 0.7355\\
\hline
\multirow{4}{*}{catster}& Original G0 & 5448197 & 0.4055 & 10.0 & 0.3935 & 281 & 1.0 & 1.0 & 1.0 & 1.0\\
& Coarse G1 & 1270670 & 0.3143 & 15.0 & 0.6867 & 293 & 0.9989 & 0.5893 & 0.5856 & 0.3908\\
& Mid G2 & 1656230 & 0.2605 & 11.0 & 0.3728 & 360 & 0.999 & 0.8647 & 0.8725 & 0.6274\\
& Fine G3 & 1463958 & 0.2693 & 14.0 & 0.2874 & 1117 & 0.999 & 0.7564 & 0.8411 & 0.4029\\
\hline
\multirow{4}{*}{bio-human2}& Original G0 & 9027024 & 0.6574 & 7.0 & 0.3124 & 2 & 1.0 & 1.0 & 1.0 & 1.0\\
& Coarse G1 & 2372498 & 0.6661 & 7.0 & 0.7442 & 15 & 0.9966 & 0.8701 & 0.8606 & 0.7391\\
& Mid G2 & 3073818 & 0.6398 & 26.0 & 0.5158 & 14 & 0.9824 & 0.8658 & 0.8816 & 0.7353\\
& Fine G3 & 2534509 & 0.6245 & 39.0 & 0.4168 & 66 & 0.9289 & 0.8838 & 0.8671 & 0.6418\\
\hline
\multirow{4}{*}{fb-penn94}& Original G0 & 1362220 & 0.2174 & 8.0 & 0.4802 & 1 & 1.0 & 1.0 & 1.0 & 1.0\\
& Coarse G1 & 351663 & 0.3282 & 16.0 & 0.9486 & 16 & 0.9959 & 0.8503 & 0.795 & 0.5678\\
& Mid G2 & 463387 & 0.1644 & 11.0 & 0.3841 & 23 & 0.9955 & 0.8929 & 0.9004 & 0.6034\\
& Fine G3 & 365588 & 0.0377 & 14.0 & 0.3044 & 122 & 0.9951 & 0.8887 & 0.9242 & -0.0852\\
\hline
\multirow{4}{*}{ca-cit-Hepth}& Original G0 & 2444798 & 0.6117 & 9.0 & 0.4066 & 74 & 1.0 & 1.0 & 1.0 & 1.0\\
& Coarse G1 & 487512 & 0.705 & 18.0 & 0.9303 & 86 & 0.9884 & 0.8417 & 0.8383 & 0.7466\\
& Mid G2 & 875329 & 0.4934 & 13.0 & 0.3731 & 111 & 0.9934 & 0.9083 & 0.9394 & 0.8114\\
& Fine G3 & 722204 & 0.21 & 16.0 & 0.2503 & 279 & 0.993 & 0.8346 & 0.9464 & -0.0399\\
\hline
\multirow{4}{*}{livemocha}& Original G0 & 2193083 & 0.0582 & 6.0 & 0.3557 & 1 & 1.0 & 1.0 & 1.0 & 1.0\\
& Coarse G1 & 636920 & 0.0442 & 12.0 & 0.4493 & 3 & 0.9975 & 0.887 & 0.9072 & 0.4764\\
& Mid G2 & 869150 & 0.0379 & 10.0 & 0.2922 & 8 & 0.9977 & 0.9004 & 0.9121 & 0.4915\\
& Fine G3 & 556710 & 0.0156 & 11.0 & 0.2886 & 1375 & 0.9976 & 0.7712 & 0.8772 & 0.3806\\
\hline
\multirow{4}{*}{fb-texas84}& Original G0 & 1590651 & 0.1974 & 7.0 & 0.383 & 1 & 1.0 & 1.0 & 1.0 & 1.0\\
& Coarse G1 & 374658 & 0.2892 & 16.0 & 0.9212 & 16 & 0.9969 & 0.8596 & 0.8242 & 0.5696\\
& Mid G2 & 574831 & 0.1314 & 9.0 & 0.3053 & 5 & 0.995 & 0.9354 & 0.9392 & 0.6643\\
& Fine G3 & 521925 & 0.0519 & 12.0 & 0.2385 & 29 & 0.9954 & 0.9405 & 0.9576 & 0.0799\\
\hline
\multirow{4}{*}{livejournal}& Original G0 & 34681189 & 0.3538 & 21.0 & 0.7481 & 1 & 1.0 & 1.0 & 1.0 & 1.0\\
& Coarse G1 & 13560479 & 0.4654 & 72.0 & 0.9983 & 1683 & 0.9999 & 0.854 & 0.8116 & 0.7515\\
& Mid G2 & 13419647 & 0.3936 & 42.0 & 0.8016 & 7070 & 0.9998 & 0.9057 & 0.8722 & 0.7631\\
& Fine G3 & 8227627 & 0.021 & 30.0 & 0.7194 & 316906 & 0.9999 & 0.6687 & 0.727 & 0.3658\\
\hline
\multirow{4}{*}{gplus}& Original G0 & 12238285 & 0.5165 & 6.0 & 0.4703 & 1 & 1.0 & 1.0 & 1.0 & 1.0\\
& Coarse G1 & 3585750 & 0.5445 & 14.0 & 0.8898 & 15 & 0.9987 & 0.9105 & 0.9045 & 0.5858\\
& Mid G2 & 2954045 & 0.418 & 12.0 & 0.3838 & 18 & 0.9983 & 0.903 & 0.8793 & 0.5658\\
& Fine G3 & 3341129 & 0.1509 & 19.0 & 0.2596 & 905 & 0.9983 & 0.7877 & 0.8846 & -0.2603\\
\hline
\multirow{4}{*}{bio-mouse}& Original G0 & 14461095 & 0.5308 & 12.0 & 0.6164 & 97 & 1.0 & 1.0 & 1.0 & 1.0\\
& Coarse G1 & 4577389 & 0.5961 & 21.0 & 0.894 & 105 & 0.9915 & 0.9392 & 0.9517 & 0.7224\\
& Mid G2 & 4145431 & 0.2775 & 13.0 & 0.556 & 132 & 0.9959 & 0.9282 & 0.9353 & 0.6548\\
& Fine G3 & 4062434 & 0.0587 & 14.0 & 0.5155 & 400 & 0.9958 & 0.912 & 0.955 & 0.0846\\
\hline
\multirow{4}{*}{cit-patent}& Original G0 & 16518947 & 0.0919 & 26.0 & 0.8107 & 3627 & 1.0 & 1.0 & 1.0 & 1.0\\
& Coarse G1 & 5755324 & 0.1632 & 61.0 & 0.9335 & 43758 & 0.9998 & 0.7947 & 0.775 & 0.7306\\
& Mid G2 & 3404490 & 0.13 & 57.0 & 0.9728 & 631405 & 0.9999 & 0.5758 & 0.6444 & 0.5906\\
& Fine G3 & 5023228 & 0.0073 & 39.0 & 0.8385 & 235519 & 0.9999 & 0.6784 & 0.7426 & 0.5445\\
\hline
\multirow{4}{*}{bio-human1}& Original G0 & 12323680 & 0.6303 & 8.0 & 0.3831 & 17 & 1.0 & 1.0 & 1.0 & 1.0\\
& Coarse G1 & 2834679 & 0.6557 & 18.0 & 0.8029 & 19 & 0.9862 & 0.9009 & 0.9513 & 0.7399\\
& Mid G2 & 4013787 & 0.3264 & 9.0 & 0.3923 & 22 & 0.994 & 0.9109 & 0.905 & 0.7086\\
& Fine G3 & 3870373 & 0.0584 & 11.0 & 0.3281 & 78 & 0.9943 & 0.89 & 0.9287 & 0.2066\\
\hline
\multirow{4}{*}{foursquare}& Original G0 & 3214986 & 0.2209 & 4.0 & 0.4074 & 1 & 1.0 & 1.0 & 1.0 & 1.0\\
& Coarse G1 & 1127851 & 0.1688 & 36.0 & 0.9402 & 18 & 0.9997 & 0.7374 & 0.8795 & 0.8653\\
& Mid G2 & 765900 & 0.1944 & 47.0 & 0.9383 & 366 & 0.9992 & 0.4901 & 0.7788 & 0.7851\\
& Fine G3 & 1083343 & 0.0356 & 14.0 & 0.5735 & 10008 & 0.9997 & 0.3581 & 0.7376 & 0.7258\\
\hline
\end{tabular}


==> results/multiscale_results/ms_result_table_new.tex <==
\begin{tabular}{ |l|l|l|l|l|l|l|l|l|l|l| }
	\hline
	Graph Name & Graphs & \multicolumn{9}{|c|}{ Properties } \\
	\hline
	- & - & $|E|$ & CC & D & Q & $\Gamma$ & $C_B$($\rho$) & $PR_{\rho}$ & $DC_{\rho}$ & $CC_{\rho}$\\
	\hline \multirow{4}{*}{fb-indiana}& G0 & 1.3M & 0.21 & 8.0 & 0.45 & 1 & 1.0 & 1.0 & 1.0 & 1.0\\
& G1 & 361.4K & 0.31 & 13.0 & 0.93 & 18 & 1.0 & 0.84 & 0.83 & 0.64\\
& G2 & 349.8K & 0.14 & 10.0 & 0.34 & 8 & 0.99 & 0.89 & 0.89 & 0.57\\
& G3 & 402.7K & 0.04 & 12.0 & 0.3 & 37 & 0.99 & 0.93 & 0.95 & 0.03\\
\hline
\multirow{4}{*}{bio-human2}& G0 & 9.0M & 0.66 & 7.0 & 0.31 & 2 & 1.0 & 1.0 & 1.0 & 1.0\\
& G1 & 2.4M & 0.67 & 7.0 & 0.74 & 15 & 1.0 & 0.87 & 0.86 & 0.74\\
& G2 & 3.1M & 0.64 & 26.0 & 0.52 & 14 & 0.98 & 0.87 & 0.88 & 0.74\\
& G3 & 2.5M & 0.62 & 39.0 & 0.42 & 66 & 0.93 & 0.88 & 0.87 & 0.64\\
\hline
\multirow{4}{*}{bio-human1}& G0 & 12.3M & 0.63 & 8.0 & 0.38 & 17 & 1.0 & 1.0 & 1.0 & 1.0\\
& G1 & 2.8M & 0.66 & 18.0 & 0.8 & 19 & 0.99 & 0.9 & 0.95 & 0.74\\
& G2 & 4.0M & 0.33 & 9.0 & 0.39 & 22 & 0.99 & 0.91 & 0.91 & 0.71\\
& G3 & 3.9M & 0.06 & 11.0 & 0.33 & 78 & 0.99 & 0.89 & 0.93 & 0.21\\
\hline
\multirow{4}{*}{flickr}& G0 & 2.3M & 0.09 & 9.0 & 0.67 & 83 & 1.0 & 1.0 & 1.0 & 1.0\\
& G1 & 921.0K & 0.15 & 35.0 & 0.91 & 144 & 1.0 & 0.6 & 0.62 & 0.78\\
& G2 & 496.1K & 0.12 & 18.0 & 0.84 & 134 & 1.0 & 0.71 & 0.73 & 0.8\\
& G3 & 634.9K & 0.04 & 25.0 & 0.55 & 5834 & 1.0 & 0.64 & 0.77 & 0.74\\
\hline
\multirow{4}{*}{fb-uf}& G0 & 1.5M & 0.22 & 8.0 & 0.44 & 1 & 1.0 & 1.0 & 1.0 & 1.0\\
& G1 & 423.4K & 0.24 & 12.0 & 0.61 & 3 & 0.99 & 0.88 & 0.88 & 0.58\\
& G2 & 425.1K & 0.16 & 11.0 & 0.37 & 15 & 1.0 & 0.9 & 0.9 & 0.6\\
& G3 & 418.9K & 0.05 & 11.0 & 0.27 & 57 & 1.0 & 0.92 & 0.95 & -0.01\\
\hline
\multirow{4}{*}{livejournal}& G0 & 34.7M & 0.35 & 21.0 & 0.75 & 1 & 1.0 & 1.0 & 1.0 & 1.0\\
& G1 & 13.6M & 0.47 & 72.0 & 1.0 & 1683 & 1.0 & 0.85 & 0.81 & 0.75\\
& G2 & 13.4M & 0.39 & 42.0 & 0.8 & 7070 & 1.0 & 0.91 & 0.87 & 0.76\\
& G3 & 8.2M & 0.02 & 30.0 & 0.72 & 316906 & 1.0 & 0.67 & 0.73 & 0.37\\
\hline
\end{tabular}



==> results/multiscale_results/sn1_weak.tex <==
\begin{tabular}{ |l|l|l|l|l|l|l|l|l|l|l| }
		\hline
		\textbf{Graph Name} & \textbf{Level} & \multicolumn{9}{|c|}{ \textbf{Properties} } \\
		\hline
		- & - & \ $|E|$ & CC & D & Q & $\Gamma$ & $C_B$($\rho$) & $PR_{\rho}$ & $DC_{\rho}$ & $CC_{\rho}$\\
		\hline \multirow{4}{*}{fb-indiana}& G0 & 1.3M & 0.21 & 8.0 & 0.44 & 1 & 1.0 & 1.0 & 1.0 & 1.0\\
& G1 & 462.2K & 0.3 & 10.0 & 0.89 & 17 & 1.0 & 0.87 & 0.84 & 0.69\\
& G2 & 519.1K & 0.28 & 20.0 & 0.69 & 25 & 0.99 & 0.88 & 0.85 & 0.7\\
& G3 & 237.4K & 0.29 & 51.0 & 0.79 & 735 & 0.99 & 0.81 & 0.85 & 0.27\\
\hline
\multirow{4}{*}{fb-texas84}& G0 & 1.6M & 0.2 & 7.0 & 0.37 & 1 & 1.0 & 1.0 & 1.0 & 1.0\\
& G1 & 558.3K & 0.26 & 11.0 & 0.8 & 10 & 1.0 & 0.9 & 0.9 & 0.68\\
& G2 & 495.7K & 0.25 & 19.0 & 0.67 & 47 & 0.99 & 0.88 & 0.83 & 0.61\\
& G3 & 270.6K & 0.24 & 31.0 & 0.69 & 971 & 0.99 & 0.82 & 0.85 & 0.19\\
\hline
\multirow{4}{*}{fb-uf}& G0 & 1.5M & 0.22 & 8.0 & 0.44 & 1 & 1.0 & 1.0 & 1.0 & 1.0\\
& G1 & 407.2K & 0.35 & 11.0 & 0.92 & 26 & 1.0 & 0.84 & 0.83 & 0.61\\
& G2 & 569.2K & 0.3 & 25.0 & 0.66 & 38 & 1.0 & 0.89 & 0.82 & 0.68\\
& G3 & 269.3K & 0.31 & 43.0 & 0.8 & 1.2K & 0.98 & 0.79 & 0.84 & 0.25\\
\hline
\multirow{4}{*}{fb-penn94}& G0 & 1.4M & 0.22 & 8.0 & 0.49 & 1 & 1.0 & 1.0 & 1.0 & 1.0\\
& G1 & 520.1K & 0.3 & 13.0 & 0.86 & 19 & 1.0 & 0.88 & 0.76 & 0.67\\
& G2 & 385.4K & 0.32 & 40.0 & 0.79 & 170 & 0.99 & 0.84 & 0.81 & 0.53\\
& G3 & 381.7K & 0.28 & 35.0 & 0.77 & 1.2K & 0.99 & 0.81 & 0.84 & 0.27\\
\hline
\multirow{4}{*}{livejournal}& G0 & 34.7M & 0.35 & 21.0 & 0.75 & 1 & 1.0 & 1.0 & 1.0 & 1.0\\
& G1 & 13.8M & 0.46 & 61.0 & 1.0 & 1.3K & 1.0 & 0.86 & 0.82 & 0.76\\
& G2 & 11.7M & 0.46 & 94.0 & 0.95 & 69.3K & 1.0 & 0.86 & 0.83 & 0.73\\
& G3 & 10.3M & 0.22 & 64.0 & 0.88 & 563.7K & 1.0 & 0.67 & 0.74 & 0.37\\
\hline
\multirow{4}{*}{gplus}& G0 & 12.2M & 0.52 & 6.0 & 0.48 & 1 & 1.0 & 1.0 & 1.0 & 1.0\\
& G1 & 3.3M & 0.55 & 13.0 & 0.91 & 34 & 1.0 & 0.91 & 0.9 & 0.59\\
& G2 & 4.7M & 0.52 & 20.0 & 0.72 & 121 & 1.0 & 0.91 & 0.89 & 0.64\\
& G3 & 2.8M & 0.41 & 62.0 & 0.71 & 3.6K & 1.0 & 0.79 & 0.85 & -0.05\\
\hline
\end{tabular}



==> results/multiscale_results/sn2_weak.tex <==
\begin{tabular}{ |l|l|l|l|l|l|l|l|l|l|l| }
		\hline
		\textbf{Graph Name} & \textbf{Level} & \multicolumn{9}{|c|}{ \textbf{Properties} } \\
		\hline
		- & - & \ $|E|$ & CC & D & Q & $\Gamma$ & $C_B$($\rho$) & $PR_{\rho}$ & $DC_{\rho}$ & $CC_{\rho}$\\
		\hline \multirow{4}{*}{flickr}& G0 & 2.3M & 0.09 & 9.0 & 0.67 & 83 & 1.0 & 1.0 & 1.0 & 1.0\\
& G1 & 915.7K & 0.14 & 35.0 & 0.92 & 140 & 1.0 & 0.6 & 0.62 & 0.78\\
& G2 & 756.4K & 0.13 & 36.0 & 0.89 & 220 & 1.0 & 0.65 & 0.69 & 0.82\\
& G3 & 603.2K & 0.17 & 49.0 & 0.84 & 10.5K & 1.0 & 0.61 & 0.72 & 0.73\\
\hline
\multirow{4}{*}{buzznet}& G0 & 2.8M & 0.25 & 5.0 & 0.31 & 1 & 1.0 & 1.0 & 1.0 & 1.0\\
& G1 & 959.7K & 0.29 & 13.0 & 0.63 & 14 & 1.0 & 0.65 & 0.86 & 0.5\\
& G2 & 670.0K & 0.3 & 23.0 & 0.67 & 51 & 1.0 & 0.63 & 0.89 & 0.5\\
& G3 & 758.1K & 0.25 & 34.0 & 0.6 & 1.1K & 1.0 & 0.57 & 0.89 & 0.35\\
\hline
\multirow{4}{*}{foursquare}& G0 & 3.2M & 0.22 & 4.0 & 0.4 & 1 & 1.0 & 1.0 & 1.0 & 1.0\\
& G1 & 1.2M & 0.17 & 32.0 & 0.94 & 23 & 1.0 & 0.69 & 0.87 & 0.86\\
& G2 & 1.2M & 0.19 & 42.0 & 0.86 & 26 & 1.0 & 0.7 & 0.87 & 0.87\\
& G3 & 1.1M & 0.22 & 32.0 & 0.76 & 7.5K & 1.0 & 0.57 & 0.81 & 0.83\\
\hline
\multirow{4}{*}{catster}& G0 & 5.4M & 0.41 & 10.0 & 0.39 & 281 & 1.0 & 1.0 & 1.0 & 1.0\\
& G1 & 1.4M & 0.31 & 12.0 & 0.78 & 296 & 1.0 & 0.71 & 0.64 & 0.42\\
& G2 & 1.1M & 0.34 & 23.0 & 0.71 & 408 & 1.0 & 0.66 & 0.55 & 0.65\\
& G3 & 969.2K & 0.26 & 38.0 & 0.75 & 2.6K & 1.0 & 0.66 & 0.7 & 0.46\\
\hline
\multirow{4}{*}{blog-catalog}& G0 & 2.1M & 0.46 & 9.0 & 0.32 & 1 & 1.0 & 1.0 & 1.0 & 1.0\\
& G1 & 453.3K & 0.48 & 10.0 & 0.81 & 19 & 1.0 & 0.8 & 0.84 & 0.5\\
& G2 & 785.3K & 0.48 & 20.0 & 0.64 & 14 & 0.99 & 0.88 & 0.92 & 0.67\\
& G3 & 660.0K & 0.46 & 19.0 & 0.64 & 509 & 0.99 & 0.75 & 0.89 & 0.41\\
\hline
\multirow{4}{*}{livemocha}& G0 & 2.2M & 0.06 & 6.0 & 0.36 & 1 & 1.0 & 1.0 & 1.0 & 1.0\\
& G1 & 817.5K & 0.07 & 12.0 & 0.66 & 6 & 1.0 & 0.9 & 0.89 & 0.59\\
& G2 & 501.2K & 0.07 & 36.0 & 0.75 & 12 & 0.99 & 0.83 & 0.85 & 0.48\\
& G3 & 414.2K & 0.05 & 28.0 & 0.68 & 1.4K & 0.99 & 0.74 & 0.86 & 0.4\\
\hline
\end{tabular}



==> results/normalized_cc_plots.tex <==
%\textbf{Clustering Coef. (Normalized)}\\
%\newpage
\footnotesize
\begin{figure}[H]
\footnotesize
\hspace{-1cm}
\begin{tabular}{m{0cm} m{.25cm} m{3.6cm} m{3.6cm} m{3.6cm}}
 & & \centering $\rho$-weak & \centering mixed & \centering $\rho$-strong \arraybackslash \\
& \raisebox{.25\height}{\rotatebox{90}{\parbox{1.9cm}{Social\\Networks 1}}} &
\includegraphics[width=\linewidth, page=4]{results/plots/normalized/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf} &
\includegraphics[width=\linewidth, page=5]{results/plots/normalized/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf} &
\includegraphics[width=\linewidth, page=6]{results/plots/normalized/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}\\
& & \multicolumn{3}{c}{\includegraphics[width=\linewidth, page=25]{results/plots/normalized/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}} \\
& \raisebox{.25\height}{\rotatebox{90}{\parbox{1.9cm}{Social\\Networks 2}}} &
\includegraphics[width=\linewidth, page=4]{results/plots/normalized/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf} &
\includegraphics[width=\linewidth, page=5]{results/plots/normalized/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf} &
\includegraphics[width=\linewidth, page=6]{results/plots/normalized/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}\\
& & \multicolumn{3}{c}{\includegraphics[width=\linewidth, page=25]{results/plots/normalized/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}} \\
& \raisebox{.25\height}{\rotatebox{90}{\parbox{1.9cm}{Citation\\Networks}}} &
\includegraphics[width=\linewidth, page=4]{results/plots/normalized/ca-cit-Hepth_codblp_cit-patent.pdf} &
\includegraphics[width=\linewidth, page=5]{results/plots/normalized/ca-cit-Hepth_codblp_cit-patent.pdf} &
\includegraphics[width=\linewidth, page=6]{results/plots/normalized/ca-cit-Hepth_codblp_cit-patent.pdf}\\
& & \multicolumn{3}{c}{\includegraphics[width=\linewidth, page=25]{results/plots/normalized/ca-cit-Hepth_codblp_cit-patent.pdf}} \\
& \raisebox{.25\height}{\rotatebox{90}{\parbox{1.9cm}{Biological\\Networks}}} &
\includegraphics[width=\linewidth, page=4]{results/plots/normalized/human1_human2_mouse.pdf} &
\includegraphics[width=\linewidth, page=5]{results/plots/normalized/human1_human2_mouse.pdf} &
\includegraphics[width=\linewidth, page=6]{results/plots/normalized/human1_human2_mouse.pdf}\\
& & \multicolumn{3}{c}{\includegraphics[width=\linewidth, page=25]{results/plots/normalized/human1_human2_mouse.pdf}} \\
\end{tabular}
\caption{Clustering Coef. (Normalized)}
\end{figure}
\normalsize




==> results/plots.tex <==
\input{unnormalized}\\

\newpage
\footnotesize
\begin{figure}
\footnotesize
\hspace{-1cm}
\begin{tabular}{m{0cm} m{.25cm} m{3.6cm} m{3.6cm} m{3.6cm}}
\multirow{8}{*}{\hspace{-2cm}\includegraphics[angle=90,page=25]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}} & &
\centering $\rho$-weak & \centering mixed & \centering $\rho$-strong \arraybackslash \\
& \raisebox{.25\height}{\rotatebox{90}{\parbox{1.9cm}{Betweenness\\centrality}}} &
\includegraphics[width=\linewidth, page=1]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf} &
\includegraphics[width=\linewidth, page=2]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf} &
\includegraphics[width=\linewidth, page=3]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}\\
& \raisebox{.25\height}{\rotatebox{90}{\parbox{1.9cm}{Clustering coeff.\\distribution}}}  &
\includegraphics[width=\linewidth, page=7]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}&
\includegraphics[width=\linewidth, page=8]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf} &
\includegraphics[width=\linewidth, page=9]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}\\
& \raisebox{.25\height}{\rotatebox{90}{\parbox{1.9cm}{Degree\\centrality}}}  &
\includegraphics[width=\linewidth, page=10]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf} &
\includegraphics[width=\linewidth, page=11]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf} &
\includegraphics[width=\linewidth, page=12]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}\\
& \raisebox{.25\height}{\rotatebox{90}{\parbox{2cm}{Diameter}}}  &
\includegraphics[width=\linewidth, page=13]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}&
\includegraphics[width=\linewidth, page=14]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf} &
\includegraphics[width=\linewidth, page=15]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}\\
& \raisebox{.25\height}{\rotatebox{90}{\parbox{2cm}{Connected\\components}}}  &
\includegraphics[width=\linewidth, page=16]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf} &
\includegraphics[width=\linewidth, page=17]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf} &
\includegraphics[width=\linewidth, page=18]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}\\
& \raisebox{.25\height}{\rotatebox{90}{\parbox{2cm}{Modularity}}}  &
\includegraphics[width=\linewidth, page=19]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}&
\includegraphics[width=\linewidth, page=20]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf} &
\includegraphics[width=\linewidth, page=21]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}\\
& \raisebox{.25\height}{\rotatebox{90}{\parbox{2cm}{PageRank}}}  &
\includegraphics[width=\linewidth, page=22]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf} &
\includegraphics[width=\linewidth, page=23]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf} &
\includegraphics[width=\linewidth, page=24]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}
\end{tabular}
\caption{Social networks.}
\end{figure}
\normalsize

\textbf{Facebook graphs, Livejournal, Gplus}\\
\Image[width=\linewidth, page=25]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}\\

\newpage
\textbf{Facebook graphs, Livejournal, Gplus}\\
\captionof{figure}{Betweenness Centrality}
\Image[width=0.3\linewidth, page=1]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=2]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=3]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{c. strong}\\
\captionof{figure}{Clustering coef.}
\Image[width=0.3\linewidth, page=4]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=5]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=6]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{c. strong}\\
\captionof{figure}{Clustering Coefficient Distribution}
\Image[width=0.3\linewidth, page=7]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=8]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=9]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{c. strong}\\
\captionof{figure}{Degree Centrality}
\Image[width=0.3\linewidth, page=10]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=11]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=12]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{c. strong}\\
\captionof{figure}{Diameter}
\Image[width=0.3\linewidth, page=13]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=14]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=15]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{c. strong}\\
\captionof{figure}{Components}
\Image[width=0.3\linewidth, page=16]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=17]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=18]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{c. strong}\\
\captionof{figure}{Modularity}
\Image[width=0.3\linewidth, page=19]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=20]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=21]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{c. strong}\\
\captionof{figure}{Pagerank}
\Image[width=0.3\linewidth, page=22]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=23]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=24]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{c. strong}\\
\Image[width=\linewidth, page=25]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}\\

\textbf{Social Networks}\\
\captionof{figure}{Betweenness Centrality}
\Image[width=0.3\linewidth, page=1]{results/plots/regular/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=2]{results/plots/regular/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=3]{results/plots/regular/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{c. strong}\\
\captionof{figure}{Clustering coef.}
\Image[width=0.3\linewidth, page=4]{results/plots/regular/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=5]{results/plots/regular/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=6]{results/plots/regular/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{c. strong}\\
\captionof{figure}{Clustering Coefficient Distribution}
\Image[width=0.3\linewidth, page=7]{results/plots/regular/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=8]{results/plots/regular/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=9]{results/plots/regular/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{c. strong}\\
\captionof{figure}{Degree Centrality}
\Image[width=0.3\linewidth, page=10]{results/plots/regular/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=11]{results/plots/regular/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=12]{results/plots/regular/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{c. strong}\\
\captionof{figure}{Diameter}
\Image[width=0.3\linewidth, page=13]{results/plots/regular/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=14]{results/plots/regular/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=15]{results/plots/regular/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{c. strong}\\
\captionof{figure}{Components}
\Image[width=0.3\linewidth, page=16]{results/plots/regular/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=17]{results/plots/regular/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=18]{results/plots/regular/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{c. strong}\\
\captionof{figure}{Modularity}
\Image[width=0.3\linewidth, page=19]{results/plots/regular/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=20]{results/plots/regular/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=21]{results/plots/regular/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{c. strong}\\
\captionof{figure}{Pagerank}
\Image[width=0.3\linewidth, page=22]{results/plots/regular/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=23]{results/plots/regular/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=24]{results/plots/regular/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{c. strong}\\
\Image[width=\linewidth, page=25]{results/plots/regular/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}\\

\textbf{Citation Networks}\\
\captionof{figure}{Betweenness Centrality}
\Image[width=0.3\linewidth, page=1]{results/plots/regular/ca-cit-Hepth_codblp_cit-patent.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=2]{results/plots/regular/ca-cit-Hepth_codblp_cit-patent.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=3]{results/plots/regular/ca-cit-Hepth_codblp_cit-patent.pdf}{c. strong}\\
\captionof{figure}{Clustering coef.}
\Image[width=0.3\linewidth, page=4]{results/plots/regular/ca-cit-Hepth_codblp_cit-patent.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=5]{results/plots/regular/ca-cit-Hepth_codblp_cit-patent.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=6]{results/plots/regular/ca-cit-Hepth_codblp_cit-patent.pdf}{c. strong}\\
\captionof{figure}{Clustering Coefficient Distribution}
\Image[width=0.3\linewidth, page=7]{results/plots/regular/ca-cit-Hepth_codblp_cit-patent.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=8]{results/plots/regular/ca-cit-Hepth_codblp_cit-patent.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=9]{results/plots/regular/ca-cit-Hepth_codblp_cit-patent.pdf}{c. strong}\\
\captionof{figure}{Degree Centrality}
\Image[width=0.3\linewidth, page=10]{results/plots/regular/ca-cit-Hepth_codblp_cit-patent.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=11]{results/plots/regular/ca-cit-Hepth_codblp_cit-patent.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=12]{results/plots/regular/ca-cit-Hepth_codblp_cit-patent.pdf}{c. strong}\\
\captionof{figure}{Diameter}
\Image[width=0.3\linewidth, page=13]{results/plots/regular/ca-cit-Hepth_codblp_cit-patent.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=14]{results/plots/regular/ca-cit-Hepth_codblp_cit-patent.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=15]{results/plots/regular/ca-cit-Hepth_codblp_cit-patent.pdf}{c. strong}\\
\captionof{figure}{Components}
\Image[width=0.3\linewidth, page=16]{results/plots/regular/ca-cit-Hepth_codblp_cit-patent.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=17]{results/plots/regular/ca-cit-Hepth_codblp_cit-patent.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=18]{results/plots/regular/ca-cit-Hepth_codblp_cit-patent.pdf}{c. strong}\\
\captionof{figure}{Modularity}
\Image[width=0.3\linewidth, page=19]{results/plots/regular/ca-cit-Hepth_codblp_cit-patent.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=20]{results/plots/regular/ca-cit-Hepth_codblp_cit-patent.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=21]{results/plots/regular/ca-cit-Hepth_codblp_cit-patent.pdf}{c. strong}\\
\captionof{figure}{Pagerank}
\Image[width=0.3\linewidth, page=22]{results/plots/regular/ca-cit-Hepth_codblp_cit-patent.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=23]{results/plots/regular/ca-cit-Hepth_codblp_cit-patent.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=24]{results/plots/regular/ca-cit-Hepth_codblp_cit-patent.pdf}{c. strong}\\
\Image[width=\linewidth, page=25]{results/plots/regular/ca-cit-Hepth_codblp_cit-patent.pdf}\\

\textbf{Biological Networks}\\
\captionof{figure}{Betweenness Centrality}
\Image[width=0.3\linewidth, page=1]{results/plots/regular/human1_human2_mouse.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=2]{results/plots/regular/human1_human2_mouse.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=3]{results/plots/regular/human1_human2_mouse.pdf}{c. strong}\\
\captionof{figure}{Clustering coef.}
\Image[width=0.3\linewidth, page=4]{results/plots/regular/human1_human2_mouse.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=5]{results/plots/regular/human1_human2_mouse.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=6]{results/plots/regular/human1_human2_mouse.pdf}{c. strong}\\
\captionof{figure}{Clustering Coefficient Distribution}
\Image[width=0.3\linewidth, page=7]{results/plots/regular/human1_human2_mouse.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=8]{results/plots/regular/human1_human2_mouse.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=9]{results/plots/regular/human1_human2_mouse.pdf}{c. strong}\\
\captionof{figure}{Degree Centrality}
\Image[width=0.3\linewidth, page=10]{results/plots/regular/human1_human2_mouse.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=11]{results/plots/regular/human1_human2_mouse.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=12]{results/plots/regular/human1_human2_mouse.pdf}{c. strong}\\
\captionof{figure}{Diameter}
\Image[width=0.3\linewidth, page=13]{results/plots/regular/human1_human2_mouse.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=14]{results/plots/regular/human1_human2_mouse.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=15]{results/plots/regular/human1_human2_mouse.pdf}{c. strong}\\
\captionof{figure}{Components}
\Image[width=0.3\linewidth, page=16]{results/plots/regular/human1_human2_mouse.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=17]{results/plots/regular/human1_human2_mouse.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=18]{results/plots/regular/human1_human2_mouse.pdf}{c. strong}\\
\captionof{figure}{Modularity}
\Image[width=0.3\linewidth, page=19]{results/plots/regular/human1_human2_mouse.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=20]{results/plots/regular/human1_human2_mouse.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=21]{results/plots/regular/human1_human2_mouse.pdf}{c. strong}\\
\captionof{figure}{Pagerank}
\Image[width=0.3\linewidth, page=22]{results/plots/regular/human1_human2_mouse.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=23]{results/plots/regular/human1_human2_mouse.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=24]{results/plots/regular/human1_human2_mouse.pdf}{c. strong}\\
\Image[width=\linewidth, page=25]{results/plots/regular/human1_human2_mouse.pdf}\\

\input{normalized}\\
\textbf{Facebook graphs, Livejournal, Gplus}\\
\captionof{figure}{Betweenness Centrality}
\Image[width=0.3\linewidth, page=1]{results/plots/normalized/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=2]{results/plots/normalized/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=3]{results/plots/normalized/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{c. strong}\\
\captionof{figure}{Clustering coef.}
\Image[width=0.3\linewidth, page=4]{results/plots/normalized/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=5]{results/plots/normalized/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=6]{results/plots/normalized/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{c. strong}\\
\captionof{figure}{Clustering Coefficient Distribution}
\Image[width=0.3\linewidth, page=7]{results/plots/normalized/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=8]{results/plots/normalized/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=9]{results/plots/normalized/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{c. strong}\\
\captionof{figure}{Degree Centrality}
\Image[width=0.3\linewidth, page=10]{results/plots/normalized/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=11]{results/plots/normalized/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=12]{results/plots/normalized/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{c. strong}\\
\captionof{figure}{Diameter}
\Image[width=0.3\linewidth, page=13]{results/plots/normalized/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=14]{results/plots/normalized/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=15]{results/plots/normalized/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{c. strong}\\
\captionof{figure}{Components}
\Image[width=0.3\linewidth, page=16]{results/plots/normalized/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=17]{results/plots/normalized/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=18]{results/plots/normalized/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{c. strong}\\
\captionof{figure}{Modularity}
\Image[width=0.3\linewidth, page=19]{results/plots/normalized/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=20]{results/plots/normalized/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=21]{results/plots/normalized/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{c. strong}\\
\captionof{figure}{Pagerank}
\Image[width=0.3\linewidth, page=22]{results/plots/normalized/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=23]{results/plots/normalized/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=24]{results/plots/normalized/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}{c. strong}\\
\Image[width=\linewidth, page=25]{results/plots/normalized/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}\\

\textbf{Social Networks}\\
\captionof{figure}{Betweenness Centrality}
\Image[width=0.3\linewidth, page=1]{results/plots/normalized/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=2]{results/plots/normalized/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=3]{results/plots/normalized/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{c. strong}\\
\captionof{figure}{Clustering coef.}
\Image[width=0.3\linewidth, page=4]{results/plots/normalized/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=5]{results/plots/normalized/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=6]{results/plots/normalized/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{c. strong}\\
\captionof{figure}{Clustering Coefficient Distribution}
\Image[width=0.3\linewidth, page=7]{results/plots/normalized/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=8]{results/plots/normalized/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=9]{results/plots/normalized/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{c. strong}\\
\captionof{figure}{Degree Centrality}
\Image[width=0.3\linewidth, page=10]{results/plots/normalized/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=11]{results/plots/normalized/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=12]{results/plots/normalized/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{c. strong}\\
\captionof{figure}{Diameter}
\Image[width=0.3\linewidth, page=13]{results/plots/normalized/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=14]{results/plots/normalized/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=15]{results/plots/normalized/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{c. strong}\\
\captionof{figure}{Components}
\Image[width=0.3\linewidth, page=16]{results/plots/normalized/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=17]{results/plots/normalized/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=18]{results/plots/normalized/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{c. strong}\\
\captionof{figure}{Modularity}
\Image[width=0.3\linewidth, page=19]{results/plots/normalized/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=20]{results/plots/normalized/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=21]{results/plots/normalized/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{c. strong}\\
\captionof{figure}{Pagerank}
\Image[width=0.3\linewidth, page=22]{results/plots/normalized/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=23]{results/plots/normalized/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=24]{results/plots/normalized/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}{c. strong}\\
\Image[width=\linewidth, page=25]{results/plots/normalized/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}\\

\textbf{Citation Networks}\\
\captionof{figure}{Betweenness Centrality}
\Image[width=0.3\linewidth, page=1]{results/plots/normalized/ca-cit-Hepth_codblp_cit-patent.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=2]{results/plots/normalized/ca-cit-Hepth_codblp_cit-patent.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=3]{results/plots/normalized/ca-cit-Hepth_codblp_cit-patent.pdf}{c. strong}\\
\captionof{figure}{Clustering coef.}
\Image[width=0.3\linewidth, page=4]{results/plots/normalized/ca-cit-Hepth_codblp_cit-patent.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=5]{results/plots/normalized/ca-cit-Hepth_codblp_cit-patent.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=6]{results/plots/normalized/ca-cit-Hepth_codblp_cit-patent.pdf}{c. strong}\\
\captionof{figure}{Clustering Coefficient Distribution}
\Image[width=0.3\linewidth, page=7]{results/plots/normalized/ca-cit-Hepth_codblp_cit-patent.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=8]{results/plots/normalized/ca-cit-Hepth_codblp_cit-patent.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=9]{results/plots/normalized/ca-cit-Hepth_codblp_cit-patent.pdf}{c. strong}\\
\captionof{figure}{Degree Centrality}
\Image[width=0.3\linewidth, page=10]{results/plots/normalized/ca-cit-Hepth_codblp_cit-patent.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=11]{results/plots/normalized/ca-cit-Hepth_codblp_cit-patent.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=12]{results/plots/normalized/ca-cit-Hepth_codblp_cit-patent.pdf}{c. strong}\\
\captionof{figure}{Diameter}
\Image[width=0.3\linewidth, page=13]{results/plots/normalized/ca-cit-Hepth_codblp_cit-patent.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=14]{results/plots/normalized/ca-cit-Hepth_codblp_cit-patent.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=15]{results/plots/normalized/ca-cit-Hepth_codblp_cit-patent.pdf}{c. strong}\\
\captionof{figure}{Components}
\Image[width=0.3\linewidth, page=16]{results/plots/normalized/ca-cit-Hepth_codblp_cit-patent.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=17]{results/plots/normalized/ca-cit-Hepth_codblp_cit-patent.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=18]{results/plots/normalized/ca-cit-Hepth_codblp_cit-patent.pdf}{c. strong}\\
\captionof{figure}{Modularity}
\Image[width=0.3\linewidth, page=19]{results/plots/normalized/ca-cit-Hepth_codblp_cit-patent.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=20]{results/plots/normalized/ca-cit-Hepth_codblp_cit-patent.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=21]{results/plots/normalized/ca-cit-Hepth_codblp_cit-patent.pdf}{c. strong}\\
\captionof{figure}{Pagerank}
\Image[width=0.3\linewidth, page=22]{results/plots/normalized/ca-cit-Hepth_codblp_cit-patent.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=23]{results/plots/normalized/ca-cit-Hepth_codblp_cit-patent.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=24]{results/plots/normalized/ca-cit-Hepth_codblp_cit-patent.pdf}{c. strong}\\
\Image[width=\linewidth, page=25]{results/plots/normalized/ca-cit-Hepth_codblp_cit-patent.pdf}\\

\textbf{Biological Networks}\\
\captionof{figure}{Betweenness Centrality}
\Image[width=0.3\linewidth, page=1]{results/plots/normalized/human1_human2_mouse.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=2]{results/plots/normalized/human1_human2_mouse.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=3]{results/plots/normalized/human1_human2_mouse.pdf}{c. strong}\\
\captionof{figure}{Clustering coef.}
\Image[width=0.3\linewidth, page=4]{results/plots/normalized/human1_human2_mouse.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=5]{results/plots/normalized/human1_human2_mouse.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=6]{results/plots/normalized/human1_human2_mouse.pdf}{c. strong}\\
\captionof{figure}{Clustering Coefficient Distribution}
\Image[width=0.3\linewidth, page=7]{results/plots/normalized/human1_human2_mouse.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=8]{results/plots/normalized/human1_human2_mouse.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=9]{results/plots/normalized/human1_human2_mouse.pdf}{c. strong}\\
\captionof{figure}{Degree Centrality}
\Image[width=0.3\linewidth, page=10]{results/plots/normalized/human1_human2_mouse.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=11]{results/plots/normalized/human1_human2_mouse.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=12]{results/plots/normalized/human1_human2_mouse.pdf}{c. strong}\\
\captionof{figure}{Diameter}
\Image[width=0.3\linewidth, page=13]{results/plots/normalized/human1_human2_mouse.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=14]{results/plots/normalized/human1_human2_mouse.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=15]{results/plots/normalized/human1_human2_mouse.pdf}{c. strong}\\
\captionof{figure}{Components}
\Image[width=0.3\linewidth, page=16]{results/plots/normalized/human1_human2_mouse.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=17]{results/plots/normalized/human1_human2_mouse.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=18]{results/plots/normalized/human1_human2_mouse.pdf}{c. strong}\\
\captionof{figure}{Modularity}
\Image[width=0.3\linewidth, page=19]{results/plots/normalized/human1_human2_mouse.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=20]{results/plots/normalized/human1_human2_mouse.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=21]{results/plots/normalized/human1_human2_mouse.pdf}{c. strong}\\
\captionof{figure}{Pagerank}
\Image[width=0.3\linewidth, page=22]{results/plots/normalized/human1_human2_mouse.pdf}{a. weak} \,
\Image[width=0.3\linewidth, page=23]{results/plots/normalized/human1_human2_mouse.pdf}{b. mixed} \,
\Image[width=0.3\linewidth, page=24]{results/plots/normalized/human1_human2_mouse.pdf}{c. strong}\\
\Image[width=\linewidth, page=25]{results/plots/normalized/human1_human2_mouse.pdf}\\


==> results/regular_cc_plots.tex <==
%\textbf{Clustering Coef. (Unnormalized)}\\
%\newpage
\footnotesize
\begin{figure}[H]
\footnotesize
\hspace{-1cm}
\begin{tabular}{m{0cm} m{.25cm} m{3.6cm} m{3.6cm} m{3.6cm}}
 & & \centering $\rho$-weak & \centering mixed & \centering $\rho$-strong \arraybackslash \\
& \raisebox{.25\height}{\rotatebox{90}{\parbox{1.9cm}{Social\\Networks 1}}} &
\includegraphics[width=\linewidth, page=4]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf} &
\includegraphics[width=\linewidth, page=5]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf} &
\includegraphics[width=\linewidth, page=6]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}\\
& & \multicolumn{3}{c}{\includegraphics[width=\linewidth, page=25]{results/plots/regular/fb-indiana_fb-uf_fb-texas84_fb-penn94_gplus_lj.pdf}} \\
& \raisebox{.25\height}{\rotatebox{90}{\parbox{1.9cm}{Social\\Networks 2}}} &
\includegraphics[width=\linewidth, page=4]{results/plots/regular/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf} &
\includegraphics[width=\linewidth, page=5]{results/plots/regular/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf} &
\includegraphics[width=\linewidth, page=6]{results/plots/regular/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}\\
& & \multicolumn{3}{c}{\includegraphics[width=\linewidth, page=25]{results/plots/regular/flickr_foursquare_catster_buzznet_blogcatalog_livemocha.pdf}} \\
& \raisebox{.25\height}{\rotatebox{90}{\parbox{1.9cm}{Citation\\Networks}}} &
\includegraphics[width=\linewidth, page=4]{results/plots/regular/ca-cit-Hepth_codblp_cit-patent.pdf} &
\includegraphics[width=\linewidth, page=5]{results/plots/regular/ca-cit-Hepth_codblp_cit-patent.pdf} &
\includegraphics[width=\linewidth, page=6]{results/plots/regular/ca-cit-Hepth_codblp_cit-patent.pdf}\\
& & \multicolumn{3}{c}{\includegraphics[width=\linewidth, page=25]{results/plots/regular/ca-cit-Hepth_codblp_cit-patent.pdf}} \\
& \raisebox{.25\height}{\rotatebox{90}{\parbox{1.9cm}{Biological\\Networks}}} &
\includegraphics[width=\linewidth, page=4]{results/plots/regular/human1_human2_mouse.pdf} &
\includegraphics[width=\linewidth, page=5]{results/plots/regular/human1_human2_mouse.pdf} &
\includegraphics[width=\linewidth, page=6]{results/plots/regular/human1_human2_mouse.pdf}\\
& & \multicolumn{3}{c}{\includegraphics[width=\linewidth, page=25]{results/plots/regular/human1_human2_mouse.pdf}} \\
\end{tabular}
\caption{Clustering Coef. (Unnormalized)}
\end{figure}
\normalsize



